Modular Self-Supervision for Document-Level Relation Extraction

Extracting relations across large text spans has been relatively underexplored in NLP, but it is particularly important for high-value domains such as biomedicine, where obtaining high recall of the latest findings is crucial for practical applications. Compared to conventional information extraction confined to short text spans, document-level relation extraction faces additional challenges in both inference and learning. Given longer text spans, state-of-the-art neural architectures are less effective and task-specific self-supervision such as distant supervision becomes very noisy. In this paper, we propose decomposing document-level relation extraction into relation detection and argument resolution, taking inspiration from Davidsonian semantics. This enables us to incorporate explicit discourse modeling and leverage modular self-supervision for each sub-problem, which is less noise-prone and can be further refined end-to-end via variational EM. We conduct a thorough evaluation in biomedical machine reading for precision oncology, where cross-paragraph relation mentions are prevalent. Our method outperforms prior state of the art, such as multi-scale learning and graph neural networks, by over 20 absolute F1 points. The gain is particularly pronounced among the most challenging relation instances whose arguments never co-occur in a paragraph.

==> sections/experiments.tex <==
\section{Experiments}

There are two prominent tasks to validate our approach: DocRED~\cite{yao-etal-2019-docred}
and Biomedical Machine Reading~\cite{quirk-poon-2017-distant,peng-etal-2017-cross,wang-poon-2018-deep,jia-etal-2019-document}.
We compare them in \Cref{sec:dataset-comparison} and find that
while both tasks aim to accelerate document-level relation extraction, 
the relation scope in DocRED is often within a few sentences,
and its documents on average contain around 200 words with no paragraph boundaries.\footnote{DocRED is created using the intro section in Wikipedia, not the entire article.}  
In contrast, the relation scope in Biomedical Machine Reading is expanded over dozens of sentences and across several paragraphs.
Its documents are the entire article text, containing thousands of words with explicit paragraph boundaries.
Therefore, we choose Biomedical Machine Reading to validate our approach.
See \Cref{sec:dataset-comparison} for the detailed comparison.

\begin{table}[!t]
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{}} & \multirow{2}{*}{Train} & \multirow{2}{*}{Dev} & \multicolumn{2}{c}{Test} \\ \cmidrule(l){4-5} 
 &  &  & CKB & CKB$^\diamond$\\ \midrule
\textbf{Source} & DS & DS & MC & MC\\
\textbf{Documents} & 15828 & 3948 & 430 & 391 \\
\textbf{Uniq. facts} & 631 & 522 & 1566 & 325 \\
\textbf{Positive ex.} & 49119 & 12133 & 1904 & 332 \\
\textbf{Negative ex.} & 247671 & 57755 & 15840 & 11790 \\
\multicolumn{4}{l}{\hspace{-0.62em}\textbf{In each document}}  &  \\
~~Avg words & 3179 & 3217  & 5480 & 5576 \\
~~Avg sents & 101 & 102 & 171 & 174 \\
~~Avg paras & 25 & 26 & 39 & 39 \\
\multicolumn{4}{l}{\hspace{-0.62em}\textbf{Between each positive entity pair}}  &  \\
~~Avg words & 480 & 497 & 162 & 718 \\
~~Avg sents & 14 & 15 & 5 & 22 \\
~~Avg paras & 3 & 3 & 1 & 4 \\ \bottomrule
\end{tabular}
\caption{Biomedical Machine Reading data statistics. Both training and dev sets are distantly supervised (DS). The test set is manually curated (MC).
The distance between each positive entity pair is measured using their closest mention pair.}
\label{tab:data-statisitcs}
\end{table}


\subsection{Biomedical Machine Reading}
\label{sec:dataset}
Biomedical Machine Reading is a task to
extract drug-mutation interactions from biomedical literature.
Unlike previous work on cross-sentence relation extraction~\cite{peng-etal-2017-cross,jia-etal-2019-document},
we consider a common yet underexplored situation
where the given drug and mutation may never co-occur in the same paragraph. 
\citet{jia-etal-2019-document} has shown that
these cross-paragraph drug-mutation pairs account for a significant portion of the overall relational facts,
and in the real world they are often of high value to molecular tumor boards.

For training and development, we use documents from the PubMed Central Open Access Subset (PMC-OA)\footnote{\url{www.ncbi.nlm.nih.gov/pmc/}}.
Distant supervision is from three knowledgebases with hand-curated drug-mutation facts:
CIVIC\footnote{\url{civicdb.org/home}}, GDKD~\cite{dienstmann2015database}, and OncoKB~\cite{chakravarty2017oncokb}.
We randomly split the generated data into training and development sets and ensure no overlap of documents.
\Cref{tab:data-statisitcs} summarizes their statistics.
We use them to train and tune baselines and our approach.

For test, we use CKB CORE\texttrademark, a public subset of the Clinical Knowledgebase (CKB; \citealt{patterson2016clinical})\footnote{\url{ckbhome.jax.org}},
as our gold-standard test set.
CKB CORE\texttrademark~contains high-quality document-level annotations of drug-mutation interactions,
which are manually curated from PubMed articles by The Jackson Laboratory (JAX), an NCI-designated cancer center.
CKB has minimal overlap with the three KBs used for training and dev.
To avoid contamination, we remove CKB entries whose documents are used in our training and dev sets.
See \Cref{tab:data-statisitcs} for statistics.
We also consider a subset of our test data (denoted as CKB$^\diamond$),
where drug-mutation pairs never co-occur in the same paragraph.
While CKB$^\diamond$ contains 332/1904 (17.4\%) positive examples of the entire test set,
its negative example rate is overwhelming.
To our knowledge, CKB CORE\texttrademark~is the only manually curated data that contains a significant portion of cross-paragraph relational facts.

\subsection{Implementation Details}
Our system is implemented using PyTorch~\cite{pytorch}.
We incorporate early stopping to identify the best checkpoint for relation component based on the dev performance. 
We set the maximal segment length to derive relation evidences to 2 consecutive sentences. 
The resolution component is self-trained with 8 iterations.
All model encoders are initialized with the pretrained PubMedBERT parameters~\cite{pubmedbert},
and are fine-tuned using the AdamW optimizer~\cite{loshchilov2017decoupled}. 
We report the detailed hyperparameter setttings in \Cref{sec:hyperparameters}. 
We follow \citet{wang-poon-2018-deep,jia-etal-2019-document} to conduct standard data preprocessing and entity linking.


\begin{table*}[!t]
\centering
\begin{tabular}{@{}C{2cm}lR{2.2cm}R{2.5cm}R{2.5cm}@{}}
\toprule
Test Set & System & Precision (\%) & Recall (\%) & F1 (\%)~~ \\ \midrule
\multirow{4}{*}{CKB} & All Positive & 10.73 {\footnotesize $\pm$0.00} & 100.00 {\footnotesize $\pm$0.00} & 19.38 {\footnotesize $\pm$0.00}~~ \\  
& Multiscale~\cite{jia-etal-2019-document} & 21.17 {\footnotesize$\pm$0.50} & 59.27 {\footnotesize$\pm$0.16} & 31.19 {\footnotesize$\pm$0.53}~~ \\
 & GAIN~\cite{zeng-etal-2020-double} & 42.26 {\footnotesize$\pm$2.03} & 33.48 {\footnotesize$\pm$1.47} & 37.28 {\footnotesize$\pm$0.18}~~ \\
 & Modular SSL (Ours) & 49.89 {\footnotesize$\pm$0.27} & 71.54 {\footnotesize$\pm$0.28} & 59.78 {\footnotesize$\pm$0.13}~~ \\ \midrule
\multirow{4}{*}{CKB$^\diamond$} & All Positive & 2.74 {\footnotesize $\pm$0.00} & 100.00 {\footnotesize $\pm$0.00} & 5.33 {\footnotesize $\pm$0.00}~~ \\  
 & Multiscale~\cite{jia-etal-2019-document} & 4.73 {\footnotesize$\pm$0.18} & 42.80 {\footnotesize$\pm$0.91} & 8.51 {\footnotesize$\pm$0.29}~~ \\
 & GAIN~\cite{zeng-etal-2020-double} & 7.99 {\footnotesize$\pm$0.42} & 13.66 {\footnotesize$\pm$1.35} & 10.04 {\footnotesize$\pm$0.36}~~ \\
 & Modular SSL (Ours) & 22.62 {\footnotesize$\pm$0.08} & 46.05 {\footnotesize$\pm$0.37} & 30.34 {\footnotesize$\pm$0.11}~~ \\ \bottomrule
\end{tabular}
\caption{Comparison of different systems on CKB and CKB$^\diamond$. We run each system 3 times with different random seeds and report their average and standard deviation.}
\label{tab:main-results}
\end{table*}


\subsection{Results}
\label{sec:results}
We compare our modular self-supervised learning approach (\textbf{Modular SSL}) with the following baselines:
(a) \textbf{All Positive} is a simple baseline which always predicts positive for any given example.
(b) \textbf{Multiscale}~\cite{jia-etal-2019-document} is an entity-centric approach.
It achieves the state of the art on Biomedical Machine Reading
by combining mention-level representations learned over different discourse units and subrelation hierarchy. 
(c) \textbf{GAIN}~\cite{zeng-etal-2020-double} constructs heterogeneous mention-level graphs
and utilizes graph convolutional network~\cite{kipf2017semi} to model the interactions among intra- and inter-sentence mentions.
GAIN signifcantly improves the state of the art on DocRED~\cite{yao-etal-2019-docred}.
Note that for fair comparisons, we replace the encoders in Multiscale and GAIN with the same pretrained PubMedBERT used in our approach.

\Cref{tab:main-results} shows the experiment results.
On the entire test set (CKB), our approach substantially outperforms all baselines.
It has the highest precision while maintaining considerably high recall.
Multiscale and GAIN are two representative end-to-end approaches. 
With noisy distantly supervised training data, both approaches perform mediocrely:  
Multiscale achieves relatively higher recall, and GAIN shows better precision.
% Not surprisingly, Modular (Coref+RE), the modular baseline, also has significantly lower scores compared to our approach. 
% This shows the limitation of SpanBERT~\cite{joshi-etal-2020-spanbert} in general domains, as well as
% the necessity of domain-specific self-training for the resolution component.
On the much more challenging test subset (CKB$^\diamond$), we see an amplified difference between our approach and the baselines.
All baselines fail in distinguishing hundreds of positive cross-paragraph examples from over 30 times larger negative ones.
Only Multiscale shows comparable recall with our approach,
but its precision is extremely low, minimal difference with the All Positive baseline.

In addition to the results above, we also investigate the effect of supervision quality on the performance of end-to-end approaches.
We split a half of the CKB test set to fine-tune a BERT-based Multiscale model, and evaluate it against the other half of the CKB test set.
No significant improvement is observed, which demonstrates the efficiency of our approaches under limited supervision.


\begin{table}[!ht]
\centering
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
 & Prec. & Recall & F1 \\ \midrule
Full model & 22.62 & 46.05 & 30.34 \\
\makecell[bl]{$\triangleright$~Replace relation component\\~~~with all positive function} & 13.73 & 66.06 & 22.73 \\ 
\makecell[bl]{$\triangleright$~Replace resolution component\\~~~with Multi-Sieve Pass} & 10.99 & 42.77 & 17.48 \\
\makecell[bl]{$\triangleright$~Replace resolution component\\~~~with SpanBERT Coref} & 60.19 & 1.48 & 2.89 \\
\makecell[bl]{$\triangleright$~Remove noisy data filter}& 26.09 & 38.76 & 26.35 \\  \bottomrule
\end{tabular}
\caption{Ablation study on CKB$^\diamond$.}
\label{tab:ablation-study}
\end{table}

\subsection{Ablation Study}
We conduct ablation study on CKB$^\diamond$ in \Cref{tab:ablation-study}.
To show the contribution of relation component, we replace it with a function which always predicts positive for any relation evidence.
On one hand, this replacement allows us to see the recall upper bound of our approach (66.06\%).
On the other hand, the drastic precision drop reveals that the relation component succeeds at discarding a significant number of negative examples.
Next, we investigate the contribution of resolution component by
replacing it with two alternates: an unsupervised coreference resolution framework, Multi-Sieve Pass~\cite{raghunathan-etal-2010-multi,lee-etal-2011-stanfords},
and the state-of-the-art coreference resolution model, SpanBERT~\cite{joshi-etal-2020-spanbert}.
Both replacements result in a significant performance drop, which shows the advantage of our resolution component.
Through extensions to Multi-Sieve Pass and self-training,
the resolution component combines the unsupervised framework and the neural coreference resolution model, leading to a substantial improvement.
Lastly, we remove the noisy data filter when training the relation component.
While precision slightly increases, both F1 and recall drop significantly.

\subsection{Analysis}

\noindent\textbf{Self-training}
As described in \Cref{algo:learn-resolution-component},
at each iteration of self-training, new pseudo labels are added to the training data to update the parameters of resolution component,
which in turns generates more pseudo labels.
Since there is no gold resolution labels, we evaluate the resolution component at each iteration on the end task CKB$^\diamond$.
We use an all-positive function as the relation component
such that we can remove potential variance from the relation component and focus on evaluating the resolution component. 
\Cref{fig:resolution-component-learning} shows the performance improvement over the self-training process.
We see moderate increases in F1 and precision with steady decreasing of their variance.
More importantly, recall is improved significantly over the process,
which provides higher upper bound for our full model evaluation.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/res-comp-learn.pdf}
    \caption{The performance improvement of resolution component on CKB$^\diamond$ over the self-training process.}
    \label{fig:resolution-component-learning}
\end{figure}

\noindent\textbf{Segment Length}
In \Cref{sec:formulation}, we formulate the relation evidence as a template derived from a consecutive text segment,
and set the maximal segment length to 2 sentences in the experiments.
\Cref{fig:seg-len-eff} shows the results on CKB$^\diamond$ when different maximal segment lengths are chosen.
As we increase the maximal segment length, we observe that recall increases while precision drops, resulting a notable drop of F1.
Setting the maximal length to 2 sentences allows us to keep a relatively high recall without losing too much precision.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/seg-len-eff.pdf}
    \caption{The effect of different maximal segment lengths (i.e. the number of sentences).}
    \label{fig:seg-len-eff}
\end{figure}

\begin{table}[!ht]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
 & Prec. & Recall & F1 \\ \midrule
Our approach & & & \\
 ~~w/ PubMedBERT & 22.62 & 46.05 & 30.34 \\
 ~~w/ SpanBERT & 21.91 & 38.76 & 27.99 \\
 \bottomrule
\end{tabular}
\caption{Comparison of our approach based different pretrained encoders on CKB$^\diamond$.}
\label{tab:bert-comp}
\end{table}

\noindent\textbf{Pretrained Encoders}
With domain-specific pretraining, PubMedBERT shows the state-of-art performance on biomedical natural language processing~\cite{pubmedbert}. 
Therefore, we choose to initialize encoders in our approach with PubMedBERT. 
In \Cref{tab:bert-comp}, we compare PubMedBERT with SpanBERT~\cite{joshi-etal-2020-spanbert},
another pretrained language model that outperforms the original BERT on a variety of tasks on the general domain.
Owing to the domain-specific vocabulary and pretraining, PubMedBERT shows better results with a substantial gain on recall. 


\noindent\textbf{Error Analysis}
\Cref{tab:ablation-study} shows the recall upper bound is 66.06\%,
meaning that about 34\% relations are beyond the reach of our the current setup.
After analyzing false negative samples, we find that most of them can be categorized into three groups:
(a) Relation evidences are only available from text segments that exceeds the maximal segment length. 
While increasing the maximal segment length can improve recall. it will also cause a precision drop (\Cref{fig:seg-len-eff}).
(b) Key resolution links between target entities and entities in the relation evidence are missing.
We can improve the resolution component to alleviate this issue, and leave it for future work.
(c) No direct relation evidence can be found in the text.
Oftentimes these relations are expressed in figures, tables, or supplements, beyond the scope of our extraction.

As for precision, it still has room for improvement, especially on CKB$^\diamond$.
According to our analysis on false positive samples,
most of the time the relation component make correct classification, and errors are from the resolution component.
The most common error is caused by exact string match, 
which classifies two \emph{gene} mentions as coreference
but in fact they are described in different experiments with focus on different variants.
The resolution component also make some mistakes in classifying \emph{is-a} and \emph{part-of} relations.
In most of the remaining cases, they are actually true relations but are excluded by curators due to additional curation criteria.

==> sections/inference.tex <==
\section{Inference}

To find out whether an entity pair $(e_1, e_2)$ in a document $D$ has the relation $R(e_1, e_2)$, we adopt a two-stage process.
First, given a set of entity mentions $M$ in $D$, 
the resolution component $P(I(m,n)|D,\bm{\psi})$ predicts the resolution link between each mention pair $(m,n)$, 
which is used to construct the document-level resolution graph.
Second, we search the document-level resolution graph for any mention pair $(a_i, b_i)$ that satisfies the following conditions:
(1) $I(a_i, e_1)\wedge I(b_i,e_2)$; (2) $a_i$ and $b_i$ co-occur in a $k$-sentence segment $S_i(a_i,b_i)$.
Given the segment $S_i(a_i,b_i)$,
if the relation evidence $Z_i$ is true according the prediction of relation component $P(Z_i|S_i(a_i,b_i),\bm{\theta})$,
then the entity pair $(e_1,e_2)$ has the relation $R(e_1, e_2)$.


==> sections/introduction.tex <==
Relation extraction plays a vital role in a variety of general-domain NLP applications,
and it also shows great potentials in precision medicine~\cite{bahcall2015precision}.
%high-value domains, such as accelerating manual curation in precision oncology~\cite{bahcall2015precision,quirk-poon-2017-distant}.
Due to the advent of big data and success of deep learning, 
recent work begins to expand their research from intra-sentential relations to inter-sentential relations
\cite{li2016biocreative,quirk-poon-2017-distant,wu2019renet,yao-etal-2019-docred}.
% relation extraction from single sentences to multiple sentences.
However, the scope of relation is still mostly limited to a few consecutive sentences, leaving a significant amount of document-level relations underexplored.
While a few attempts~\cite{jia-etal-2019-document} have been made to extract document-level $n$-ary relations,  
they require at least each entity pair (i.e. subrelations) co-occur in the same paragraph,
and are unable to extract cross-paragraph entity pairs.

An example cross-paragraph entity pair (\textcolor{drug}{\emph{\textbf{cobimetinib}}}, \textcolor{variant}{\emph{\textbf{p.K57T}}}) is shown in \Cref{fig:motivating-example}.
To answer "\emph{whether \textcolor{drug}{\textbf{cobimetinib}} can be used to treat tumors with the \textcolor{variant}{\textbf{p.K57T}} mutant}",
one needs to read not only the two paragraph with the entities but also another paragraph that contains a supportive evidence (underlined)
but does not explicitly mention either of the entities.
Maximizing recall of such high-value medical findings could mean a life-and-death difference to patients.  
Nevertheless, it is challenging to learn to automatically extract them as
we will show in \Cref{sec:results}:
% (a) Manual annotations are quite expensive and laborious for relational facts across paragraph boundaries.
% Only few annotations are created for evaluation not for training.
(a) self-supervision (e.g. distant supervision) becomes extremely noisy as we expand the scope of relation across paragraphs; 
(b) existing end-to-end approaches to relation extraction struggle with very long textual spans.




Inspired by Davidsonian semantics~\cite{Davidson1967-DAVTLF},
we propose to decompose document-level relation extraction into relation detection and argument resolution,
which enables us to incorporate explicit discourse modeling and leverage modular self-supervision for each sub-problem.
As a result, the supervision signals become less noise-prone and they can be further refined end-to-end via variational EM.
We validate our approach thoroughly in biomedical machine reading for precision oncology,
where cross-paragraph relations are especially prevalent.
Compared to prior state of the art such as multiscale learning~\cite{jia-etal-2019-document} and graph neural networks~\cite{zeng-etal-2020-double},
our approach substantially improves the performance by over 20\% F1.
The gain is even more pronounced among the most challenging relation instances whose arguments never co-occur in the same paragraph.
In addition, we investigate the contributions of each module in our approach.
We also show that the modular approach provides more insights behind the predictions than end-to-end neural architectures,
which is of great importance to the real-word applications such as assisted curation in precision medicine~\cite{bahcall2015precision,quirk-poon-2017-distant}.


==> sections/learning.tex <==
\section{Learning}\label{sec:learning}
In this section,
we describe how to leverage distant supervision and variational EM to learn parameters for our model components,
when human annotations are not available.

\subsection{Distant Supervision for Relation Component}
Distant supervision uses an existing knowledge base (KB) and unlabeled text to generate training examples,
which can be extremely noisy for entities that are \emph{not} in the same paragraph.
However, for our relation evidence model, since we restrict the input to a consecutive text segment,
we can still leverage distant supervision to generate training examples.

Specifically, if a entity pair $(a,b)$ is known to have the relation in the KB,
we generate positive examples by  (i) extracting all text segments from a document in which the entity mention pair $(a, b)$ co-occur,
(ii) prepending a \texttt{[CLS]} token to each segment,
(iii) and then replacing mentions $(a,b)$ with corresponding special tokens \texttt{[X]} and \texttt{[Y]}.
We randomly sample co-occurring entity mention pairs not known to have the relation to generate negative examples.
To further reduce the noise in generated examples,
we add two restrictions:
(1) we require that a segment contains a limited number of sentences and should not span across paragraphs;
(2) we only keep positive examples for an entity pair if the number of extracted segments from a document is above a threshold.
We will shown in Sec. that these restrictions lead to better performance.

The generated examples are divided into training and development sets.
During training, a weighted sampler is used to generate mini batches so that the overall positive and negative training samples are balanced.
Parameters $\bm{\theta}$ in $P(Z_i|S_i(a_i,b_i),\bm{\theta})$ are learned via minimization of cross-entropy loss.
We train the model until the best performance is achieved on the dev set.

\subsection{Variational EM for Resolution Component}
Learning the resolution component involves finding parameters $\bm{\psi}$ and 
mention pair resolution links $\textbf{I}=\{I(m_1,n_1),...,I(m_i,n_i),...\}$ which are likely under the posterior distribution
$P(\bm{\psi},\textbf{I}|D)$.
We approximate the posterior using a simple factored representation.
Our variational approximation takes the following form:
\begin{equation}
    Q(\bm{\psi},\textbf{I})=\left( \prod_i q_i(I(m_i,n_i)) \right)\delta(\bm{\psi})
\end{equation}
Inspired by \citet{haghighi-klein-2010-coreference},
we use a mean field approach to update each of the RHS factors in turn to minimize the KL-divergence
between the current variational posterior and the true model posterior.

\noindent\textbf{Updating parameters} $\delta(\bm{\psi})$:
This factor places point estimates on a single value, just as in hard EM.
Updating it involves finding the value which maximizes the model (expected) log-likelihood under other factors.
Given the variational posteriors $\{q_i(\cdot)\}$ for mention resolution links,
$\delta(\bm{\psi})$ is a point estimate and is updated with:
\begin{equation}
    \delta(\bm{\psi})=\argmax_{\bm{\psi}} \mathbb{E}_{Q_{-\delta}}\ln{P(\bm{\psi},\textrm{I}|D)}
\end{equation}
where $Q_{-\delta}$ denotes all factors of the variational approximation except for the factor being updated.

\noindent\textbf{Updating resolution links} $\{q_i(I(m_i,n_i))\}$:
Each mention resolution link factor $q_i(I(m_i,n_i))$ maintains a soft approximation,
and is updated with the standard mean field form:
\begin{equation}
    q_i(I(m_i,n_i))\propto\exp\{\mathbb{E}_{Q_{-q_i}}\ln{P(\bm{\psi},\textrm{I}|D)}\}
\end{equation}
Since there is no direct supervision, it is impractical to learn all mention resolution links $\textbf{I}=\{...,I(m_i,n_i),...\}$ at once.
We instead introduce a curriculum learning algorithm as described in \Cref{algo:learn-resolution-component}.
Given a set of entity mentions $M$ in document $D$, we first initialize \textsc{seed\_links} between mentions
using high-precision resolution models (e.g. exact string match).
If two entities have a linked mention pair,
we add distant supervised links (\textsc{ds\_links}) to their other mention pairs that co-occur in a sentence.
With \textsc{seed\_links} and \textsc{ds\_links},  we alternately update parameters $\delta^t(\bm{\psi})$ and learn new resolution links $\Delta$, holding approximations to the other fixed.
These newly learned links are used to generate more distant supervised links, 
and to existing links for the next iteration.
The details of \textsc{seed\_links} and \textsc{ds\_links} are provided in Appendices.

\begin{algorithm}[!t]
\SetAlgoCaptionSeparator{}
\SetAlCapNameFnt{\small}
\SetAlCapFnt{\small}
\DontPrintSemicolon
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Document $D$ and entity mentions $M$.}
\Output{Learned parameters $\delta^*(\bm{\psi})$ and mention resolution links $\textbf{I}^*$.}
$\textbf{I}^0\leftarrow \textsc{seed\_links}(M\times M)$\;
$\textbf{I}^0\leftarrow \textbf{I}^0\cup \textsc{ds\_links}(\textbf{I}^0, M\times M)$\;
\For{$t=1:T$}{
    $\delta^t(\bm{\psi})\leftarrow\argmax_{\bm{\psi}}\mathbb{E}_{Q_{-\delta}}\ln{P(\bm{\psi},\textrm{I}^{t-1}|D)}$\;
    $\Delta\leftarrow\varnothing$\;
    \For{$(m_i,n_i) \in M\times M-\textrm{\bf I}^{t-1}$}{
        $\widetilde{\textbf{I}}\leftarrow \textbf{I}^{t-1}\cup\{I(m_i,n_i)\}$\;
        $q_i\propto\exp\{\mathbb{E}_{Q_{-q_i}}\ln{P(\bm{\psi},\widetilde{\textbf{I}}|D)}\}$\;
        \uIf{$q_i> \text{threshold}$}{
            $\Delta\leftarrow\Delta\cup\{I(m_i,n_i)\}$\;
        }
    }
    $\textbf{I}^t\leftarrow\textbf{I}^{t-1}\cup\Delta$\;
    $\textbf{I}^t\leftarrow \textbf{I}^t\cup \textsc{ds\_links}(\textbf{I}^t, M\times M)$\;
}
\Return $\delta^*(\bm{\psi})=\delta^t(\bm{\psi}), \textbf{I}^*=\textbf{I}^t$ \;
\caption{Resolution Component Learning\label{algo:learn-resolution-component}}
\end{algorithm}


==> sections/model.tex <==
\section{Model}
Rather than relying on a monolithic network to extract document-level relations in an end-to-end manner,
we assemble our model using specialized modules, akin to \citet{andreas2016neural}.
These modules are specialized in relation detection and argument resolution respectively.
\Cref{fig:modular-network} illustrates the assembly of our modular network for document-level \emph{ternary} relation extraction,
where we compose \emph{binary} \textcolor{relation-classification}{subrelation detection} modules for ternary relation detection,
and apply \textcolor{argument-resolution}{argument resolution} modules separately for each argument. 




\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/modular-network.pdf}
    \caption{Assembly of our modular network.
    Modules in \textcolor{relation-classification}{blue} are specialized in subrelation detection. 
    Modules in \textcolor{argument-resolution}{green} are specialized in argument resolution.
    The subrelation module $R_{23}$ is not used in this case.}
    \label{fig:modular-network}
\end{figure}


\subsection{Subrelation Detection}
We decompose the $n$-ary relation $R$ into binary subrelations $R_{ij}$ ($1\leq i,j\leq n$).\footnote{
Subrelations of other arities are also possible.}
Given a discourse unit $d_{ij}$ that contains entity mentions $x_i$ and $x_j$,
the subrelation detection module computes the following probability of $R_{ij}$ as below:
\begin{equation}
    P(\exists e.R_{ij}(e,x_i,x_j)|d_{ij},x_i,x_j;\bm{\theta}_{ij})
\end{equation}
where $\bm{\theta}_{ij}$ are learned parameters.

The module architecture is illustrated in \Cref{fig:model}(a).
Motivated by the superior contextual modeling capabilities of transformer-based models~\cite{transformer},
we utilize a pre-trained transformer encoder~\cite{pubmedbert} and fine-tune it for subrelation detection.
The module input is a discourse unit where a \texttt{[CLS]} token is prepended.
We replace mentions $x_i$ and $x_j$ with special tokens \texttt{[X$_i$]} and \texttt{[X$_j$]},
to prevent the module from overfitting to memorizing the mentions.
The last-layer hidden state $\bm{h}_\texttt{[CLS]}$ is passed to a feed-forward classifier to compute the probability: 
\begin{equation}
    \text{classifier}(\bm{h})=\text{sigmoid}(\text{MLP}(\bm{h}))
\end{equation}
where MLP is a multilayer perceptron, the details of which are given in the Appendix.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/model.pdf}
    \caption{Architecture of modules for
    \textcolor{relation-classification}{\bf subrelation classification} and \textcolor{argument-resolution}{\bf argument resolution}
    used in our network.}
    \label{fig:model}
\end{figure*}

\subsection{Argument Resolution}
The core of argument resolution is classify whether two entity mentions have one of the semantic relations, such as \emph{coreference} and \emph{is-a} relations. 
Instead of building the whole argument resolution module from scratch,
we utilize an unsupervised coreference system
and extend it by incorporating a neural component,
which is self-trained for improving coverage of the semantic relations.

\begin{equation}
    P(I_i(m_i,x_i)|D,m_i,x_i,\bm{\phi}_i)
\end{equation}

The unsupervised coreference system is a multi-sieve pass system~\cite{raghunathan-etal-2010-multi,lee-etal-2011-stanfords}.
It applies tiers of deterministic resolution models one at a time from highest to lowest precision,
to classify whether two mentions corefer.
For example, the first sieve (i.e., highest precision) requires an exact string match between two mentions,
whereas the last one (i.e., lowest precision) implements pronominal coreference resolution.
Each tier builds on predictions of previous tiers in the sieve, guaranteeing
that stronger features are given precedence over weaker ones.\footnote{We refer the reader to \citet{raghunathan-etal-2010-multi,lee-etal-2011-stanfords} for full details.}

We extend this system by replacing a core sieve, Precise Constructs, with a neural model.
Precise Constructs use a set of hand-crafted syntactic features to link two mentions
(e.g., appositive, relative pronoun, predicate nominative).
While Precise Constructs are highly precise, their coverage is relatively low, and adding new features requires high expertise.
We replace them with a neural model which we will show captures more syntactic patterns while remaining highly precise.
Concretely, for two mentions $(m,n)$, 
we adopt a BERT-based model to compute $P(I(m,n)|D,\bm{\psi})$.
The architecture is similar to the one used in \citet{joshi-etal-2020-spanbert} for coreference resolution.
An example is shown in \Cref{fig:model}(b): given two mentions \emph{PIK3CA mutation} and \emph{H1047R},
the model encodes the context of two mentions into hidden states.
For each mention span, the model averages last-layer hidden states of mention tokens to generate a contextual representation.
Contextual representations of two mentions are then passed to a pairwise feed-forward network to compute the probability. 

Our resolution component utilizes the extended multi-sieve pass system to construct document-level resolution graphs
and derives resolution evidences for mention pairs in each document.

Lastly, our approach combines relation and resolution components to compute joint probability of relation and resolution evidences in \Cref{eq:model}. 
With a search over all choices of $S_i(a_i,b_i)$ in $D$,
our approach not only is capable of computing the target relation probability $P(R(d,v))$ in \Cref{eq:formulation},
but also provides evidences $Z_i,X_i,Y_i$ to support the prediction.
These evidences are especially important for assisted curation.


==> sections/problem_formulation.tex <==
\section{Problem Formulation}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/formulation.pdf}
    \caption{Problem Formulation.}
    \label{fig:formulation}
\end{figure*}

\label{sec:formulation}
Let $m_1, ..., m_n$ be entity mentions in a document $D$. 
The goal of document-level $n$-ary relation extraction ($n\ge 2$) is to classify whether an $n$-ary relation $R$ holds for $m_1, ..., m_n$ in $D$, i.e.,
\begin{equation}
R(m_1,...,m_n)
\end{equation}

In this paper, we decompose it into two types of sub-problems: Relation Detection and Argument Resolution,
which is illustrated in \Cref{fig:formulation}.

\noindent\textbf{Relation Detection} is to classify whether the event of $R$ is triggered in $D$. 
We represent relation detection in Davidsonian semantics~\cite{Davidson1967-DAVTLF}:
\begin{equation}
\label{eq:relation-detection}
    \exists e.[A_1(e,x_1)\wedge...\wedge A_n(e,x_n)]
\end{equation}
where the event variable $e$ is a \emph{reification} of the $R$ event.  
Variables $x_1,...,x_n$ are arguments of $R$.
The subscript $i$ in $x_i$ and $A_i$ implies its role in the $n$-ary relation. 
The Davidsonian approach enables a decomposition of the relation $R$ into subrelations over subsets of entities.
Each subrelation is more likely to be expressed in a single discourse unit (e.g., a few consecutive sentences).
An example is underlined in \Cref{fig:formulation}, where the discourse unit
"\emph{Expression of the \textbf{MAP2K1 mutants} ... remained sensitive to \textbf{MEK inhibitors}}" expresses
$\exists e.[A_1(e, x_1)\wedge A_3(e, x_3)]$,
which is a binary relation between the drugs "\emph{MEK inhibitors}" and the mutations \emph{"MAP2K1 mutants"}.
The binary relation is a subrelation of the more general ternary treating relation $R$ among (\emph{drug}, \emph{gene}, \emph{mutation}).

\noindent\textbf{Argument Resolution} for each entity mention $m_i$ is
to classify whether we can substitute the argument $x_i$ in $A_i$ for $m_i$.
We denote argument resolution between $m_i$ and $x_i$ as a binary relation $I_i(m_i, x_i)$.
$I_i$ has the following property:
\begin{equation}
    \exists e.[I_i(m_i, x_i)\wedge A_i(e,x_i)\rightarrow A_i(e,m_i)]
\end{equation}
There are several semantic relations that validate argument resolution, including \emph{coreference} and \emph{is-a} relations.
For instance, in the underlined sentence in \Cref{fig:formulation},
we can substitute "\emph{MAP2K1 mutants}"  for "\emph{p.K57T}" and the resulted statement is still true.
This is because we infer from the document that "\emph{p.K57T is a kind of MAP2K1 mutant}" (i.e. the \emph{is-a} relation).

Since \emph{coreference} and \emph{is-a} are both transitive relations, and \emph{coreference} is symmetric,
we have the following additional properties regarding $I_i$:
\begin{align}
    I_i(a,b)\wedge I_i(b,c)\rightarrow I_i(a,c)\\
    I_i(a,b)\wedge \emph{coref}(c,b)\rightarrow I_i(a,c)
\end{align}
Using these properties, we can derive $I_i$ relations between entities across longer text spans.
For example, in \Cref{fig:formulation}, $I_i$(\emph{p.K57T}, \emph{MAP2K1 mutants}) is derived from 
$I_i$(\emph{p.K57T}, \emph{MAP2K1 mutations}) and \emph{coref}(\emph{MAP2K1 mutations}, \emph{MAP2K1 mutants}).

Argument resolution enables us to incorporate explicit discourse modeling.
Similar ideas have been explored by \citet{koch-etal-2014-type},
who use an off-the-shelf coreference system~\cite{lee-etal-2011-stanfords} to improve distance supervision.
Later in the experiments (\Cref{sec:results}),
we will show in \Cref{tab:ablation-study} that an off-the-shelf coreference system is not enough to achieve comparable results with our approach.




==> sections/related_work.tex <==
\section{Related Work}

{\bf += Coref}
Similar ideas have been explored by \citet{koch-etal-2014-type},
who use an off-the-shelf coreference system~\cite{lee-etal-2011-stanfords} to improve distance supervision.
Later in the experiments (\Cref{sec:results}),
we will show in \Cref{tab:ablation-study} that an off-the-shelf coreference system is not enough to achieve comparable results with our approach.

\noindent\textbf{Document-level relation extraction}
Traditional relation extraction focuses on binary relational facts between entities co-occurring within a sentence~\cite{surdeanu2014overview}. 
There are also early research efforts to expand relation extraction across sentence boundaries
\cite{wick-etal-2006-learning,gerber-chai-2010-beyond,swampillai-stevenson-2011-extracting,yoshikawa2011coreference,koch-etal-2014-type,yang-mitchell-2016-joint}, most of which
rely on explicit coreference annotations or assume a single event in the document.
With the success of neural models on sentence-level relation extraction~\cite{zeng-etal-2014-relation,nguyen-grishman-2015-relation}, 
recent work begins to explore more general cross-sentence relation extraction~\cite{li2016biocreative,quirk-poon-2017-distant},
spurring a diverse array of model architecture improvements
(\citealt{peng-etal-2017-cross,verga-etal-2018-simultaneously,christopoulou-etal-2019-connecting,nan-etal-2020-reasoning}; inter alia).
However, the scope of relation extraction is still within a paragraph, 
mostly a few consecutive sentences~\cite{quirk-poon-2017-distant},
paper abstracts~\cite{wu2019renet},
or Wikipedia intro sections~\cite{yao-etal-2019-docred}.
\citet{jia-etal-2019-document} expand the scope to the entire document
and focus on more general $n$-ary relation extraction.
They decompose $n$-ary relations into subrelations,
and require each subrelation be completely contained within a sentence or a paragraph.
Unlike \citet{jia-etal-2019-document}, we go one step further to tackle relations, including subrelations,
whose arguments (entities) may never co-occur within a paragraph.

\noindent\textbf{Distant supervision}
By aligning knowledge bases with text, distant supervision automatically generates large-scale but potentially noisy labeled data
 \cite{craven1999constructing,mintz-etal-2009-distant,hoffmann-etal-2011-knowledge,riedel2010modeling}.
% A common denoising strategy applies multi-instance learning by treating mention-level labels as latent variables \cite{hoffmann-etal-2011-knowledge}.
Noise from distant supervision increases as extraction scope expands beyond single sentences, motivating a variety of indirect supervision approaches~\cite{quirk-poon-2017-distant,wang-poon-2018-deep,jia-etal-2019-document}.
Our approach differs from the previous ones by decomposing document-level relation extraction into subproblems
where distant supervision can be used to generate higher-quality labeled data.

\noindent\textbf{Self-training}
As one of the semi-supervised learning approaches~\cite{chapelle2009semi},
self-training trains a base model on a small amount of labeled data;
applies it to pseudo-label unlabeled data; and uses pseudo-labeled data to augment the labeled data
to re-trains the base model in an iterative manner.
Self-training has been shown to obtain state-of-the-art performance in image classification~\cite{yalniz2019billion},
sequence generation~\cite{He2020Revisiting}, and speech recognition~\cite{kahn2020self}.
Similar to \citet{hearst-1992-automatic,brin1998extracting,10.1145/336597.336644},
our self-training approach uses a very small number of seed patterns to do bootstrap learning.
But unlike their approaches, we jointly leverage pseudo labels and distant supervision at each iteration to augment the labeled data.  

